Capturing Label Characteristics in VAEs

We present a principled approach to incorporating labels in VAEs that captures the rich characteristic information associated with those labels. While prior work has typically conflated these by learning latent variables that directly correspond to label values, we argue this is contrary to the intended effect of supervision in VAEs-capturing rich label characteristics with the latents. For example, we may want to capture the characteristics of a face that make it look young, rather than just the age of the person. To this end, we develop the CCVAE, a novel VAE model and concomitant variational objective which captures label characteristics explicitly in the latent space, eschewing direct correspondences between label values and latents. Through judicious structuring of mappings between such characteristic latents and labels, we show that the CCVAE can effectively learn meaningful representations of the characteristics of interest across a variety of supervision schemes. In particular, we show that the CCVAE allows for more effective and more general interventions to be performed, such as smooth traversals within the characteristics for a given label, diverse conditional generation, and transferring characteristics across datapoints.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/background.tex <==
% !TEX root =  rep_vae_iclr.tex

\Glspl{VAE} \citep{kingma2013auto, rezende2014stochastic} are a powerful and flexible class of model that combine the unsupervised representation-learning capabilities of deep autoencoders \citep{hinton1994autoencoders} with generative latent-variable models---a popular tool to capture factored low-dimensional representations of higher-dimensional observations.
%
In contrast to deep autoencoders, generative models capture representations of data not as distinct values corresponding to observations, but rather as \emph{distributions} of values.
%
A generative model defines a joint distribution over observed data~\(\x\) and latent variables~\(\z\) as \(p_\theta(\x,\z) = \pz \pxz\).
%
Given a model, learning representations of data can be viewed as performing \emph{inference}---learning the \emph{posterior} distribution~\(\pzx\) that constructs the distribution of latent values for a given observation.

\Glspl{VAE} employ amortized \gls{VI} \citep{wainwright2008graphical,kingma2013auto} using the encoder and decoder of an autoencoder to transform this setup by
%
\begin{inparaenum}[i)]
\item taking the model likelihood~\(\pxz\) to be parameterized by a neural network using the \emph{decoder}, and
\item constructing an amortized variational approximation~\(\qzx\) to the (intractable) posterior~\(\pzx\) using the \emph{encoder}.
\end{inparaenum}
%
The variational approximation of the posterior enables effective estimation of the objective---maximizing the marginal likelihood---through importance sampling, to derive the \gls{ELBO} of the model as
%
\begin{align}
  \label{eq:vae}
  \log p_\theta(\x)
 =\log \E_{\qzx} \left[ \frac{p_\theta(\z, \x)}{\qzx} \right]
\geq
      \E_{\qzx} \left[ \log \frac{p_\theta(\z, \x)}{\qzx} \right]
  \equiv\mL(\x; \phi, \theta).
\end{align}
%
Given observations $\D = \{\x_1, \ldots, \x_N\}$ taken to be realizations of random variables generated from an unknown distribution $p_{\D}(\x)$, the overall objective is
% 
$\frac{1}{N} \sum_n \mL(\x_n; \theta, \phi)$.
%
Hierarchical \glspl{VAE}~\cite{sonderby2016ladder} impose a hierarchy of latent variables improving the flexibility of the approximate posterior, however we do not consider these models in this work.

\Glspl{SSVAE} \citep{kingma2014semi,maaloe2016auxiliary,siddharth2017learning} consider the setting where a subset of data $\sD\subset \mathcal{D}$ is assumed to also have corresponding \emph{labels}~\(\y\).
%
Denoting the (unlabeled) data as~\(\uD = \D \backslash \sD\),
the log-marginal likelihood is decomposed as
%
\begin{align*}
  \log p\left(\D\right)
  = \sum\nolimits_{(\x, \y) \in \sD}\log p_\theta(\x, \y) + \sum\nolimits_{\x\in \uD}\log p_\theta(\x),
\end{align*}
where the individual log-likelihoods are lower bounded by their \gls{ELBO}s.
%
Standard practice is then to treat $\y$ as a latent variable to marginalize over whenever the label is not provided.
%
More specifically, most approaches consider splitting the latent space in $\z = \{\zy,\zny\}$ and then directly fix $\zy=\y$ whenever the label is provided, such that each dimension of $\zy$ explicitly represents a predicted value of a label, with this value known exactly only for the labeled datapoints.
%
Much of the original motivation for this~\citep{kingma2014semi} was based around performing semi--supervised classification of the labels, with the encoder being used to impute the values of $\zy$ for the unlabeled datapoints.
%
However, the framework is also regularly used as a basis for learning meaningful representations and performing manipulations, exploiting the presence of the decoder to generate new datapoints after intervening on the labels via changes to $\zy$.
%
It is this latter task in which our focus will lie, and for which we show this standard formulation leads to serious pathologies.
%
Namely, our primary goal is not to improve the fidelity of generations, but instead to demonstrate how label information can be used to structure the latent space such that it encapsulates and disentangles the characteristics associated with the labels.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../rep_vae_iclr"
%%% End:


==> sections/discussion.tex <==
We have presented a novel mechanism for faithfully capturing label characteristics in \glspl{VAE}, the \acrfull{ReVAE}, which captures label characteristics explicitly in the latent space while eschewing direct correspondences between label values and latents.
%
This has allowed us to encapsulate and disentangle the \emph{characteristics} associated with labels, rather than just the label values.
%
We are able to do so without affecting the ability to perform the tasks one typically does in the (semi-)supervised setting---namely classification, conditional generation, and intervention.
%
In particular, we have shown that, not only does this lead to more effective conventional label-switch interventions, it also allows for more fine-grained interventions to be performed, such as producing diverse sets of samples consistent with an intervened label value, or performing characteristic swaps between datapoints that retain relevant features.
%
%Here we introduced a novel way of performing semi-supervised learning for generative models.
%%
%Our model does not factorise the latent space into a discrete and continuous space like \cite{kingma2014semi}, but instead keeps the latent space smooth.
%%
%This is desirable as no information-theoretic flow issues arise between the continuous and discrete latent spaces.
%%
%Furthermore, our model scales efficiently with the number of labels, and performs effectively on most of the attributes in the CelebA datasets, moreover, by using an appropriate factorisation of the classifier enforces a bottom-up influence to disentangle the supervised generative factors.
%%
%Thus allowing us to alter features of the reconstructed image by only traversing single dimensions in the latent space.
%
%Our model is agnostic to the network architectures used, and it would be interesting to see the results when used with the autoregressive architectures\cite{van2016conditional, gulrajani2016pixelvae}.

%\clearpage
%\newpage
%\section*{Broader Impact}
%\ifnum\TeXLiveVersion<2019
%\vspace*{-1ex}
%\fi
%
%Manipulating generative factors of data comes with obvious advantage such as the ability to manipulate certain characteristics without affecting others, e.g. seeing what someone will look like with a different hair color, or when wearing glasses.
%%
%However, the ability to do so on such personal and potentially sensitive features leads to serious thought into the ethical considerations about how such approaches should be used. %this \gls{ReVAE} should be used.
%%
%Moreover with the ever pressing issue of Deep-Fakes\cite{korshunov2018deepfakes} undermining the confidence of images representing a true scene, this work has the potential to stoke this problem even further.
%%
%While this concern is very real, it is purely application based and limited to photographs of people---a domain which \gls{ReVAE} certainly is not exclusively tied to.
%%
%Moreover, these issues are common to all of semi--supervised learning in deep generative models, rather than being specific to our work.
%%
%The conceptual and methodological ideas presented in the paper draw attention to how representations of denotations should be stored in latent variable models, which is potentially very useful in certain domains.
%%
%Therefore, though the aforementioned concerns should not be forgotten, we do not feel like they are a basis to avoid pursuing such avenues of research.
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "../rep_vae_iclr"
%%%% End:


==> sections/experiments.tex <==
Following our reasoning in \cref{sec:rethink} we now showcase the efficacy of \gls{ReVAE} for the three broad aims of \emph{(a) intervention}, \emph{(b) conditional generation} and \emph{(c) classification} for a variety of supervision rates, denoted by $f$.
%
Specifically, we demonstrate that \gls{ReVAE} is able to: encapsulate characteristics for each label in an isolated manner; introduce diversity in the conditional generations;
%
permit a finer control on interventions; and match traditional metrics of baseline models.
%
Furthermore, we demonstrate that no existing method is able to perform all of the above,\footnote{DIVA can perform the same tasks as \gls{ReVAE} but only with the modifications we ourselves suggest and still not to a comparable quality.} highlighting its sophistication over existing methods.
%
We compare against: M2~\citep{kingma2014semi}; MVAE~\citep{MVAE_wu_2018}; and our modified version of DIVA~\citep{ilse2019diva}.
%
See~\cref{app:diva} for details.


To demonstrate the capture of label characteristics, we consider the multi-label setting and utilise the Chexpert~\citep{irvin2019chexpert} and CelebA~\citep{liu2015faceattributes} datasets.%
%
\footnote{\gls{ReVAE} is well-suited to multi-label problems, but also works on multi-class problems. See \cref{app:multi} for results and analyses on MNIST and FashionMNIST.}
%
For CelebA, we restrict ourselves to the 18 labels which are distinguishable in reconstructions; see \cref{app:celeba} for details.
%
We use the architectures from \cite{higgins2016beta} for the encoder and decoder.
%
The label-predictive distribution $\qyz$ is defined as $\text{Ber}(\y \mid \classProbs{\zc})$ with a diagonal transformation~$\classProbs{\cdot}$ enforcing $\qyz = \prod_iq_{\varphi^i}(y_i \mid  \zc^i)$.
%
The conditional prior~$\pzy$ is then defined as \(\mathcal{N}(\zc | \regMean{\y}, \regScale{\y})\) with appropriate factorization, and has its parameters also derived through MLPs.
%
See \cref{app:implementation} for further details.

\subsection{Interventions}

If \gls{ReVAE} encapsulates characteristics of a label in a single latent (or small set of latents), then it should be able to smoothly manipulate these characteristics without severely affecting others.
%
This allows for finer control during interventions, which is not possible when the latent variables directly correspond to labels.
%
To demonstrate this, we traverse two dimensions of the latent space and display the reconstructions in \cref{fig:latent_walks}.
%
These examples indicate that \gls{ReVAE} is indeed able to smoothly manipulate characteristics. % through its encapsulation and disentangling of denotations.
%
For example, in \textbf{b)} we are able to induce varying skin tones rather than have this be a binary intervention on \texttt{\small pale\,skin}, unlike DIVA in \textbf{a)}.
%
In \textbf{c)}, the $\z_c^i$ associated with the \texttt{\small necktie} label has also managed to encapsulate information about whether someone is wearing a shirt or is bare-necked.
%
No such traversals are possible for M2 and it is not clear how one would do them for MVAE; additional results, including traversals for DIVA, are given in~\cref{app:latent_walks}.

\begin{figure}[t]
  \centering
  \def\s{\,}
  \begin{tabular}{@{}c@{\s}c@{\s}c@{\s}c@{}}
    \includegraphics[width=0.24\textwidth]{media/latent_walk_Pale_Skin_and_Young_DIVA.png}
    &\includegraphics[width=0.24\textwidth]{media/latent_walk_Pale_Skin_and_Young.png}
    &\includegraphics[width=0.24\textwidth]{media/latent_walk_Smiling_and_Wearing_Necktie.png}
    &\includegraphics[width=0.24\textwidth]{media/latent_walk_Cardiomegaly_and_Pleural_Effusion.png}\\[-2ex]
  \end{tabular}
  \caption{%
    Continuous interventions through traversal of $\z_c$.
    %
    From left to right,
    a) DIVA \texttt{\small pale\,skin} and \texttt{\small young};
    b) \gls{ReVAE} \texttt{\small pale\,skin} and \texttt{\small young};
    c) \gls{ReVAE} \texttt{\small smiling} and \texttt{\small necktie};
    d) \gls{ReVAE} \texttt{\small Pleural Effusion} and \texttt{\small Cardiomegaly}.
  }
  \label{fig:latent_walks}
  \ifnum\TeXLiveVersion<2019
  \fi
\end{figure}

\subsection{Diversity of Generations}
%
Label characteristics naturally encapsulate diversity (e.g. there are many ways to smile) which should be present in the learned representations.
%
By virtue of the structured mappings between labels and characteristic latents, and since $\zc$ is parameterized by continuous distributions, \gls{ReVAE} is able to capture diversity in representations, allowing exploration for an attribute (e.g. smile) while preserving other characteristics.
%
This is not possible with labels directly defined as latents, as only discrete choices can be made---diversity can only be introduced here by sampling from the unlabeled latent space---which necessarily affects all other characteristics.
%
To demonstrate this, we reconstruct multiple times with $\z = \{\zc \sim \pzy, \zs\}$ for a fixed $\zs$.
%
We provide qualitative results in~\cref{fig:cond_gen}.

\begin{figure}[t]
  \includegraphics[width=\textwidth]{media/cond_gen_class_q(z|x).png}
  \caption{Diverse conditional generations for \gls{ReVAE}, $\y$ is held constant along each row and each column represents a different sample for $\zc \sim p(\zc|\y)$. $\zs$ is held constant over the entire figure.}
  \label{fig:cond_gen}

\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{media/var_interventions_small.png}\\
	\includegraphics[width=0.5\textwidth]{media/var_interventions_chex.png}
	\caption{Variance in reconstructions when intervening on a single label. [Top two] CelebA, from left to right: reconstruction, { \texttt{\footnotesize bangs}, \texttt{\footnotesize eyeglasses}, \texttt{\footnotesize pale\,skin}, \texttt{\footnotesize smiling}, \texttt{\footnotesize necktie}.}. [Bottom] Chexpert: reconstruction, { \texttt{\footnotesize cardiomegaly}, \texttt{\footnotesize edema}, \texttt{\footnotesize consolidation}, \texttt{\footnotesize atelectasis}, \texttt{\footnotesize pleural\,effusion}}.}
	\label{fig:diversity}
\end{figure}

%
If several samples are taken from $\zc \sim\pzy$ when intervening on only single characteristic, the resulting variations in pixel values should be focused around the locations relevant to that characteristic, e.g. pixel variations should be focused around the neck when intervening on \texttt{necktie}.
%
To demonstrate this, we perform single interventions on each class, and take multiple samples of $\zc \sim \pzy$.
%
We then display the variance of each pixel in the reconstruction in green in~\cref{fig:diversity}, where it can be seen that generally there is only variance in the spatial locations expected.
%
Interestingly, for the class \texttt{smile} (2nd from right), there is variance in the jaw line, suggesting that the model is able capture more subtle components of variation that just the mouth.
%

\subsection{Classification}
%
To demonstrate that reparameterizing the labels in the latent space does not hinder classification accuracy, we inspect the predictive ability of \gls{ReVAE} across a range of supervision rates, given in \cref{fig:acc}.
%
It can be observed that \gls{ReVAE} generally obtains prediction accuracies slightly superior to other models.
%
We emphasize here that \gls{ReVAE}'s primary purpose is not to achieve better classification accuracies; we are simply checking that it does not harm them, which it most clearly does not.
%
\begin{table}[h]
  \centering
  \def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
  \caption{Classification accuracies.}
  {\small
    \begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\s}c@{\r}c@{\r}c@{\r}c@{}}
      \toprule
      & \multicolumn{4}{c}{CelebA} & \multicolumn{4}{c}{Chexpert}\\
      \cmidrule(r{12pt}){2-5} \cmidrule{6-9}
      Model & $f=0.004$ & $f=0.06$ & $f=0.2$ & $f=1.0$ & $f=0.004$ & $f=0.06$ & $f=0.2$ & $f=1.0$ \\
      \midrule
      \gls{ReVAE} & \textbf{0.814} & \textbf{0.866} & \textbf{0.885} & \textbf{0.901} & \textbf{0.809} & \textbf{0.792} & \textbf{0.794} & \textbf{0.826} \\
      M2 & 0.794 & 0.862 & 0.877 & 0.893 & 0.799 & 0.779 & 0.777 & 0.774 \\
      DIVA & 0.807 & 0.860 & 0.867 & 0.877 & 0.747 & 0.786 & 0.781 & 0.775 \\
      MVAE & 0.793 & 0.828 & 0.847 & 0.864 & 0.759 & 0.787 & 0.767 & 0.715 \\
      \bottomrule
    \end{tabular}
  }
  \label{fig:acc}
\end{table}

\subsection{Disentanglement of labeled and unlabeled latents}

%
If a model can correctly disentangle the label characteristics from other generative factors, then manipulating $\zs$ should not change the label characteristics of the reconstruction.
%
To demonstrate this, we perform ``characteristic swaps,'' where we first obtain $\z = \{\zc, \zs\}$ for a given image, then swap in the characteristics $\zc$ to another image before reconstructing.
%
This should apply the exact characteristics, not just the label, to the scene/background of the other image (cf. \cref{fig:swap_ex}).
%
\begin{figure}[h!]
	\centering
	\begin{tabular}{@{}c@{\,\,}c@{\,}c@{\,\,}c@{\,}c@{\,}c@{}}
		\raisebox{-.4\height}{\includegraphics[width=0.085\textwidth]{media/faces_ex.png}}
		& $\bigoplus$
		& \raisebox{-.4\height}{\includegraphics[width=0.085\textwidth]{media/style_ex.png}}
		& $\mathbf{=}$
		& \raisebox{-.4\height}{\includegraphics[width=0.085\textwidth]{media/face_swaps_ex.png}}
		& \\
		%
		\(\scriptsize \{\zc, {\color{gray}\zs}\}\) &  & \(\scriptsize\!\{{\color{gray}\zc}, \zs\}\) & & \(\scriptsize \{\zc, \zs\}\) &
	\end{tabular}
	\vspace*{-0.9\baselineskip}
	\caption{Characteristic swap, where the characteristics of the first image (\texttt{blond hair, smiling, heavy makeup, female, no necktie, no glasses} etc.) are transfered to the unlabeled characteristics of the second (\texttt{red background}  etc.).
	}
	\label{fig:swap_ex}
\end{figure}
%

Comparing \gls{ReVAE} to our baselines in~\cref{fig:denotation_swaps}, we see that \gls{ReVAE} is able to transfer the exact characteristics to a greater extent than other models.
%
Particular attention is drawn to the preservation of labeled characteristics in each row, where \gls{ReVAE} is able to preserve characteristics, like the precise skin tone and hair color of the pictures on the left.
%
We see that M2 is only able to preserve the label and not the exact characteristic, while MVAE performs very poorly, effectively ignoring the attributes entirely.
%
Our modified DIVA variant performs reasonably well, but less reliably and at the cost of reconstruction fidelity compared to \gls{ReVAE}.
%

\begin{figure}[htb]
  \centering
  \def\s{\,}
  \begin{tabular}{@{}c@{\s}c@{\s}c@{\s}c@{}}
    \multicolumn{4}{c}{unlabeled contextual attributes, $\zs$} \\
    %
    &&\includegraphics[width=0.77\textwidth]{media/styles.png}& \\[-1pt]
    %
    \rotatebox{90}{\tiny\gls{ReVAE}}
    & \includegraphics[width=0.066\textwidth]{media/faces}
    & \includegraphics[width=0.77\textwidth]{media/face_swaps_ReVAE.png}
    & \multirow{5}{0pt}{\rotatebox{90}{label characteristics, $\zc$}}\\[-1pt]
    %
    \rotatebox{90}{\tiny\quad M2}
    & \includegraphics[width=0.066\textwidth]{media/faces}
    & \includegraphics[width=0.77\textwidth]{media/face_swaps_M2.png}
    & \\[-1pt]
    %
    \rotatebox{90}{\tiny\quad DIVA}
    & \includegraphics[width=0.066\textwidth]{media/faces}
    & \includegraphics[width=0.77\textwidth]{media/face_swaps_DIVA.png}
    & \\[-1pt]
    %
    \rotatebox{90}{\tiny\quad MVAE}
    & \includegraphics[width=0.066\textwidth]{media/faces}
    & \includegraphics[width=0.77\textwidth]{media/face_swaps_MVAE.png}
    &
  \end{tabular}
  \vspace{-8pt}
  \caption{Characteristic swaps. Characteristics (\texttt{smiling, brown hair, skin tone}, etc) of the left image should be preserved along the row while background information should be preserved along the column. 
  }
  \label{fig:denotation_swaps}
  \vspace*{5pt}
\end{figure}

An ideal characteristic swap should not change the probability assigned by a pre-trained classifier between the original image and a swapped one.
%
We employ this as a quantitative measure, reporting the average difference in log probabilities for multiple swaps in~\cref{tab:swap_diff}.
%
\Gls{ReVAE} is able to preserve the characteristics to a greater extent than other models.
%
DIVA's performance is largely due to its heavier weighting on the classifier,  which adversely affects reconstructions, as seen earlier.
%

\begin{table}[h!]
  \centering
  \vspace*{-3pt}
  \def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
  \caption{Difference in log-probabilities of pre-trained classifier from denotation swaps, lower is better.}
  \vspace*{-3pt}
  {\footnotesize
    \begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\s}c@{\r}c@{\r}c@{\r}c@{}}
      \toprule
      & \multicolumn{4}{c}{CelebA} & \multicolumn{4}{c}{Chexpert}\\
      \cmidrule(r{12pt}){2-5} \cmidrule{6-9}
      Model & $f=0.004$ & $f=0.06$ & $f=0.2$ & $f=1.0$ & $f=0.004$ & $f=0.06$ & $f=0.2$ & $f=1.0$ \\
      \midrule
      \gls{ReVAE} & 1.598 & \textbf{0.838} & \textbf{0.829} & \textbf{0.766} & \textbf{1.142} & \textbf{1.221} & \textbf{1.078} & \textbf{1.084} \\
%      ALVAE & 1.726 & 1.770 & 1.633 & 1.545 & 1.770 & 1.245 & 1.263 & 1.334 \\
      M2 & 2.118 & 1.194 & 1.179 & 1.143 & 1.624 & 1.43 & 1.41 & 1.415 \\
      DIVA & \textbf{1.489} & 0.976 & 0.996 & 0.941 & 1.36 & 1.25 & 1.199 & 1.259 \\
      MVAE & 2.114 & 2.113 & 2.088 & 2.121 & 1.618 & 1.624 & 1.618 & 1.601 \\
      \bottomrule
    \end{tabular}
  }
  \label{tab:swap_diff}
  \vspace*{4pt}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../rep_vae_iclr"
%%% End:


==> sections/implementation.tex <==
\subsection{Implentation}
\paragraph{M4 Model}
For comparison, we trained a standard VAE with an additional classification loss, we refer to this model as M4.
\begin{align}
\mathcal{L}_{M4} = \sum_{\x\in\mathcal{U}}\text{ELBO}(\x) + \sum_{(\x, \y)\in\mathcal{S}}\text{ELBO}(\x) + \alpha\log \qyz.
\end{align}
Here we use $\alpha = 10^6$, and $\qyz = \text{Cat}(\y\mid\classProbs{\z})$, with $\classProbs{\cdot}$ being the same classifier architecture used in the M3 model.

\subsection{Factorisation of Supervised Generative Factors}\label{sec:disentangle}

We are able to enforce a factorisation of the supervised latent factors $\qyz = \prod_iq(y_i = i \mid z_i)$. 
%
This is achieved by constraining the classifier to be a diagonal matrix, which in turn forces the encoder to embed class information for a single class in one axis in the latent space.
%
Thus, we find we are able to achieve disentanglement of the latent supervised latent factors with little effort.
%
This model is indicated by a superscript I in the experiments.

\paragraph{Rao-Blackwellisation}

To improve the model, we can perform Rao-Blackwellisation over the discrete labels.
%
We refer to this model by a superscript RB.

==> sections/introduction.tex <==
% !TEX root =  rep_vae_iclr.tex

Learning the characteristic factors of perceptual observations has long been desired for effective machine intelligence \citep{brooks1991intelligence,bengio2013,hinton2006reducing,tenenbaum1998mapping}.
%
In particular, the ability to learn \emph{meaningful} factors---capturing human-understandable characteristics from data---has been of interest from the perspective of human-like learning \citep{tenenbaum2000separating,lake2015human} and improving decision making and generalization across tasks \citep{bengio2013,tenenbaum2000separating}.
%
% notwithstanding the inherent \emph{interpretability} endowed on such systems, relevant for issues of fairness, accountability, and trust \cite{gdpr}.

At its heart, learning meaningful representations of data allows one to not only make predictions, but critically also to \emph{manipulate} factors of a datapoint.
%
For example, we might want to manipulate the age of a person in an image.
%
Such manipulations allow for the expression of causal effects between the meaning of factors and their corresponding realizations in the data.
%
They can be categorized into conditional generation---the ability to construct whole exemplar data instances with characteristics dictated by constraining relevant factors---and intervention---the ability to manipulate just particular factors for a given data point, and subsequently affect only the associated characteristics.
%

A particularly flexible framework within which to explore the learning of meaningful representations are \glspl{VAE}, a class of deep generative models where representations of data are captured in the underlying latent variables.
%
A variety of methods have been proposed for inducing meaningful factors in this framework~\citep{kim2018disentangling,mathieu2019disentangling,mao2019neuro,kingma2014semi,siddharth2017learning,vedantam2018generative}, and it has been argued that the most effective generally exploit available labels to (partially) supervise the training process~\citep{locatello2019challenging}.
%
Such approaches aim to associate certain factors of the representation (or equivalently factors of the generative model) with the labels, such that the former encapsulate the latter---providing a mechanism for manipulation via targeted adjustments of relevant factors.
%
Prior approaches have looked to achieve this by directly associating certain latent variables with labels~\citep{kingma2014semi,siddharth2017learning,maaloe2016auxiliary}.
%
Originally motivated by the desiderata of semi--supervised classification, each label is given a corresponding latent variable of the same type (e.g.~categorical), whose value is fixed to that of the label when the label is observed and imputed by the encoder when it is not.
%


Though natural, we argue that this assumption is not just unnecessary but actively harmful from a representation-learning perspective, particularly in the context of performing manipulations.
%
To allow manipulations, we want to learn latent factors that capture the characteristic information \emph{associated} with a label, which is typically much richer than just the label value itself.
%
For example, there are
%
\begin{wrapfigure}[16]{r}{0.38\textwidth}
  \vspace*{-0.4\baselineskip}
  \centering
  \includegraphics[width=\linewidth]{media/abs_fig.png}
  \vspace*{-1.2\baselineskip}
  \caption{Manipulating label characteristics for \texttt{\scriptsize ``hair color''} and \texttt{\scriptsize ``smile''}.}
  \label{fig:abstract}
\end{wrapfigure}
%
various visual characteristics of people's faces associated with the label ``young,'' but simply knowing the label is insufficient to reconstruct these characteristics for any particular instance.
%
Learning a meaningful representation that captures these characteristics, and \emph{isolates} them from others, requires encoding more than just the label value itself.


The key idea of our work is to use labels to help capture and isolate this related characteristic information in a VAE's representation.
%
We do this by exploiting the interplay between the labels and inputs to capture more information than the labels alone convey; information that will be lost (or at least entangled) if we directly encode the label itself.
%
Specifically, we introduce the \gls{ReVAE} framework, which employs a novel \gls{VAE} formulation which captures label characteristics explicitly in the latent space.
%
For each label, we introduce a set of \emph{characteristic latents} that are induced into capturing the characteristic information associated with that label.
%
By coupling this with a principled variational objective and carefully structuring the characteristic-latent and label variables , we show that \glspl{ReVAE} successfully capture meaningful representations, enabling better performance on manipulation tasks, while matching previous approaches for prediction tasks.
%
In particular, they permit certain manipulation tasks that cannot be performed with conventional approaches, such as manipulating characteristics \emph{without} changing the labels themselves and producing \emph{multiple} distinct samples consistent with the desired intervention.
%
We summarize our contributions as follows:
\begin{compactenum}[i)]
%
\item showing how labels can be used to capture and isolate rich \emph{characteristic} information;
%
\item formulating \glspl{ReVAE}, a novel model class and objective for supervised and semi-supervised learning in \glspl{VAE} that allows this information to be captured effectively;
%
\item demonstrating \glspl{ReVAE}' ability to successfully learn meaningful representations in practice.
%
\end{compactenum}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../rep_vae_iclr"
%%% End:


==> sections/related.tex <==
% !TEX root =  rep_vae_iclr.tex

The seminal work of~\citet{kingma2014semi} was the first to consider supervision in the \glspl{VAE} setting, introducing the M2 model for semi--supervised classification which was also approach to place labels directly in the latent space.
%
The related approach of~\citet{maaloe2016auxiliary} augments the encoding distribution with an additional, unobserved latent variable, enabling better semi-supervised classification accuracies.
%
\cite{siddharth2017learning} extended the above work to automatically derive the regularised objective for models with arbitrary (pre-defined) latent dependency structures.
%
The approach of placing labels directly in the latent space was also adopted in~\cite{li2019disentangled}.
%
Regarding the disparity between continuous and discrete latent variables in the typical semi-supervised \glspl{VAE},~\cite{dupont2018learning} provide an approach to enable effective \emph{unsupervised} learning in this setting.

From a purely modeling perspective, there also exists prior work on \glspl{VAE} involving hierarchies of latent variables, exploring richer higher-order inference and issues with redundancy among latent variables both in unsupervised~\citep{ranganath2016hierarchical,zhao2017learning} and semi-supervised~\citep{maaloe2017semi,maaloe2019biva} settings.
%
In the unsupervised case, these hierarchical variables do not have a direct interpretation, but exist merely to improve the flexibility of the encoder.
%
The semi-supervised approaches extend the basic M2 model to hierarchical VAEs by incorporating the labels as an additional latent \citep[see Appendix F in][for example]{maaloe2019biva}, and hence must incorporate additional regularisers in the form of classifiers as in the case of M2.
%
Moreover, by virtue of the typical dependencies assumed between labels and latents, it is difficult to disentangle the characteristics just associated with the label from the characteristics associated with the rest of the data---something we capture using our simpler split latents (\(\zc, \zs\)).

From a more conceptual standpoint, \citet{mueller2017sequence} introduces interventions (called revisions) on \glspl{VAE} for text data, regressing to auxiliary sentiment scores as a means of influencing the latent variables.
%
This formulation is similar to \cref{eq:m3} in spirit, although in practice they employ a range of additional factoring and regularizations particular to their domain of interest, in addition to training models in stages, involving different objective terms.
%
Nonetheless, they share our desire to enforce meaningfulness in the latent representations through auxiliary supervision.

Another related approach involves explicitly treating labels as another data \emph{modality} \citep{vedantam2018generative,JMVAE_suzuki_1611,MVAE_wu_2018,shi2019mmvae}.
%
This work is motivated by the need to learn latent representations that \emph{jointly encode} data from different modalities.
%
Looking back to \cref{eq:basic-revae}, by refactoring \(p(\z \mid \y)p(\y)\) as \(p(\y \mid \z)p(\z)\), and taking \(q(\z \mid \x, \y) = \mathcal{G}(q(\z \mid \x), q(\z \mid \y))\), one derives \emph{multi-modal} \glspl{VAE}, where \(\mathcal{G}\) can construct a product~\citep{MVAE_wu_2018} or mixture~\citep{shi2019mmvae} of experts.
%
Of these, the MVAE~\citep{MVAE_wu_2018} is more closely related to our setup here, as it explicitly targets cases where alternate data modalities are labels.
%
However, they differ in that the latent representations are not structured explicitly to map to distinct classifiers, and do not explore the question of explicitly capturing the label characteristics.
%
The JLVM model of \cite{adel2018discovering} is similar to the MVAE, but is motivated from an interpretability perspective---with labels providing `side-channel' information to constrain latents.
%
They adopt a flexible normalising-flow posterior from data~\(\x\), along with a multi-component objective that is additionally regularised with the information bottleneck between data~\(\x\), latent~\(\z\), and label~\(\y\).

DIVA~\citep{ilse2019diva} introduces a similar graphical model to ours, but is motivated to learn a generalized classifier for different domains.
%
The objective is formed of a classifier which is regularized by a variational term, requiring additional hyper-parameters and preventing the ability to disentangle the representations.
%
In~\cref{app:diva} we propose some modifications to DIVA that allow it to be applied in our problem domain.
%

Tangentially to our work, similar objectives of structuring the latent space using GANs also exist~\cite{xiao2017dna, xiao2018elegant}, although they focus purely on interventions and cannot perform conditional generations, classification, or estimate likelihoods.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../rep_vae_iclr"
%%% End:


==> sections/reparam_vae.tex <==
% !TEX root =  rep_vae_iclr.tex

To correct the issues discussed in the last section, we suggest eschewing the treatment of labels as direct components of the latent space and instead employ them to condition latent variables which are designed to capture the characteristics.
%
To this end, we similarly split the latent space into two components, $\z = \{\zc, \zs\}$, but where $\zc$, the \emph{characteristic latent}, is now designed to capture the characteristics associated with labels, rather than directly encode the labels themselves.
%
In this breakdown, $\zs$ is intended only to capture information not directly associated with any of the labels, unlike $\zny$ which was still tasked with capturing the characteristic information.
%

For the purposes of exposition and purely to demonstrate how one might apply this schema, we first consider a standard \gls{VAE}, with a latent space $\z = \{\zc, \zs\}$.
%
The latent representation of the \gls{VAE} will implicitly contain characteristic information required to perform classification, however the structure of the latent space will be arranged to optimize for reconstruction and characteristic information may be \emph{entangled} between $\zc$ and $\zs$.
%
If we were now to jointly learn a classifier---from $\zc$ to $\y$---with the \gls{VAE}, resulting in the following objective:
%
\begin{align}
\label{eq:m3}
\mathcal{J}
= \sum\nolimits_{\x\in\mathcal{U}}\mL_{\acrshort{VAE}}(\x)
+ \sum\nolimits_{(\x, \y)\in\mathcal{S}}
\left(\mL_{\acrshort{VAE}}(\x)
+ \alpha \E_{\qzx} \left[\log q_\varphi(\y \mid \z_c)\right]\right),
\end{align}
%
where $\alpha$ is a hyperparameter, there will be pressure on the encoder to place characteristic information in $\zc$, which can be interpreted as a stochastic layer containing the information needed for classification \emph{and} reconstruction\footnote{Though, for convenience, we implicitly assume here, and through the rest of the paper, that the labels are categorical such that the mapping $\zc\to\y$ is a classifier, we note that the ideas apply equally well if some labels are actually continuous, such that this mapping is now a probabilistic regression.}.
%
The classifier thus acts as a tool allowing $\y$ to influence the structure of $\z$, it is this high level concept, i.e. using $\y$ to structure $\z$, that we utilize in this work.
%

However, in general, the characteristics of different labels will be \emph{entangled} within $\z_c$.
%
Though it will contain the required information, the latents will typically be uninterpretable, and it is unclear how we could perform conditional generation or interventions.
%
To \emph{disentangle} the characteristics of different labels, we further partition the latent space, such that the classification of particular labels $y^i$ only has access to particular latents $\z_c^i$ and thus
%
\(\log \qyz = \sum\nolimits_{i}\log q_{\varphi^i} (y^i \mid \z_c^i)\).
%
This has the critical effect of forcing the characteristic information needed to classify $y^i$ to be stored only in the corresponding $\z_c^i$, providing a means to encapsulate such information for each label separately.
%
We further see that it addresses many of the prior issues: there are no measure-theoretic issues as $\z_c^i$ is not discrete, diversity in interventions is achieved by sampling different $\z_c^i$ for a given label, $\z_c^i$ can be manipulated while remaining within class decision boundaries,
%
and a mismatch between $p(\z_c)$ and $q(\z_c)$ does not manifest as there is no ground truth for $q(\z_c)$.

How to conditionally generate or intervene when training with \cref{eq:m3} is not immediately obvious though.
%
However, the classifier \emph{implicitly} contains the requisite information to do this via \emph{inference} in an implied Bayesian model. %$p(\z_c | \y) \propto p(\z_c)\qyz$.
%
For example, conditional generation needs samples from $p(\z_c)$ that classify to the desired labels, e.g.~through rejection sampling.
%
See~\cref{app:m3} for further details.



\subsection{The Characteristic Capturing VAE}
%
\begin{wrapfigure}[9]{r}{0.32\textwidth}
  \vspace*{-2.3\baselineskip}
  \centering
  \scalebox{0.78}{%
    \begin{tikzpicture}[thick,font=\small]
      % nodes
      \node[obs]                                 (x)   {$\x$};
      %
      \node[latent, above left=1.6cm and 1.1cm of x] (zs)  {$\zs$};
      \node[latent, right=1cm of zs]             (zc1) {$\zc^1$};
      \node[right=5mm of zc1,anchor=center]            {\large$\ldots$};
      \node[latent, right=1cm of zc1]            (zcl) {$\zc^L$};
      %
      \node[partial-obs, above=of zc1]           (y1)  {$\y^1$};
      \node[right=5mm of y1,anchor=center]             {\large$\ldots$};
      \node[partial-obs, right=1cm of y1]        (yl)  {$\y^L$};
      % group
      \scoped[on background layer]
        \node[fit=(y1)(yl), inner sep=2mm, fill=orange!10, rounded corners=2mm] (ys) {};
      \scoped[on background layer]
        \node[fit=(zs)(zcl), inner sep=2mm, fill=purple!10, rounded corners=2mm] (z) {};
      % connections
      \draw[->] (z) to[bend right] node[midway,left] {\(\pxz\)} (x);
      \draw[->, dashed] (x) to[bend right] node[midway,right] {\(\qzx\)} (z);
      %
      \draw[->] (y1) to[bend right] (zc1);
      \draw[->, dashed] (zc1) to[bend right] (y1);
      \draw[->] (yl) to[bend right] (zcl);
      \draw[->, dashed] (zcl) to[bend right] (yl);
      % legend -- required for varphi and psi
    \end{tikzpicture}
  }
  \vspace*{-0.65\baselineskip}
  \caption{\Gls{ReVAE} graphical model.}
  \label{fig:graphical_model}
\end{wrapfigure}
%
One way to address the need for inference is to introduce a conditional generative model $p_{\psi}(\z_c\mid \y)$, simultaneously learned alongside the classifier introduced in \cref{eq:m3}, along with a prior $p(\y)$.
%
This approach, which we term the~\gls{ReVAE}, allows the required sampling for conditional generations and interventions directly.
%
Further, by persisting with the latent partitioning above, we can introduce a factorized set of generative models $p(\z_c \mid \y) = \prod_ip(\z_c^{i} \mid y^{i})$, enabling easy generation and manipulation of $\z_c^i$ individually.
%
\Gls{ReVAE} ensures that labels remain a part of the model for unlabeled datapoints, which transpires to be important for effective learning in practice.

To address the issue of learning, we perform variational inference, treating $\y$ as a partially observed auxiliary variable.
%
The final graphical model associated with our variational model is illustrated in \cref{fig:graphical_model}.
%
The \gls{ReVAE} can be seen as a way of combining top-down and bottom-up information to obtain a structured latent representation.
%
However, it is important to highlight that \gls{ReVAE} does not contain a hierarchy of latent variables.
%
Unlike a hierarchical VAE, reconstruction is performed only from $\z \sim \qzx$ \emph{without} going through the ``deeper'' $\y$, as doing so would lead to a loss of information due to the bottleneck of $\y$.
%
By enforcing each label variable to link to different characteristic-latent dimensions, we are able to isolate the generative factors corresponding to different label characteristics.
%

\subsection{Model Objective}
\label{sec:model_obj}
%
We now construct an objective function that encapsulates the model described above, by deriving a lower bound on the full model log-likelihood which factors over the supervised and unsupervised subsets as discussed in \cref{sec:background}.
%
The supervised objective can be defined as
%
\begin{equation}
  \label{eq:basic-revae}
  \log p_{\theta,\psi}(\x, \y)
  \geq \E_{q_{\varphi, \phi}(\z \mid \x, \y)} \left[
    \log \frac{\pxz p_{\psi}(\z \mid \y)p(\y)}{q_{\varphi, \phi}(\z \mid \x, \y)}
  \right] \equiv \mathcal{L}_{\acrshort{ReVAE}}(\x, \y) ,
\end{equation}
%
with $p_{\psi}(\z \mid \y) = p(\zs)p_{\psi}(\zc \mid \y)$.
%
Here, we avoid directly modeling $q_{\varphi, \phi}(\z \mid \x, \y)$;
instead leveraging the conditional independence \(\x \perp \!\!\!\! \perp \y \mid \z\), along with Bayes rule, to give
%
\begin{equation*}
  q_{\varphi, \phi}(\z \mid \x, \y)
%  = \frac{q(\y, \z \mid \x)}{\int q(\y \mid \z)q(\z \mid \x) \mathrm{d}\z}
  = \frac{\qyz\qzx}{\qyx},
  \quad
  \text{where}
  \quad \qyx= \int \qyz \qzx \mathrm{d}\z.
\end{equation*}
%
Using this equivalence in \cref{eq:basic-revae} yields (see \cref{app:elbo} for a derivation and numerical details)
%
\begin{align}
 \mathcal{L}_{\acrshort{ReVAE}}(\x, \y)
   &\!=\!
    \E_{\qzx}\!\! \left[
    \frac{q_{\varphi}(\y \mid \z)}{\qyx}
    \log \frac{\pxz p_\psi(\z \mid \y)}{\qyz \qzx}
    \right]
    \!+\! \log q_{\varphi, \phi}(\y \mid \x)
    \!+\! \log p(\y).
  \label{eq:sup-revae}
\end{align}
%
Note that a classifier term \(\log q_{\varphi, \phi}(\y \mid \x)\) falls out naturally from the derivation, unlike previous models (e.g.~\cite{kingma2014semi,siddharth2017learning}).
%
Not placing the labels directly in the latent space is crucial for this feature.
%
When defining latents to directly correspond to labels, observing both~\(\x\) and~\(\y\) \emph{detaches} the mapping \(q_{\varphi, \phi}(\y \mid \x)\) between them, resulting in the parameters (\(\varphi, \phi\)) not being learned---motivating addition of an explicit (weighted) classifier.
%
Here, however, observing both~\(\x\) and~\(\y\) does not detach any mapping, since they are always connected via an unobserved random variable~\(\z_c\), and hence do not need additional terms.
%
From an implementation perspective, this classifier strength can be increased, we experimented with this, but found that adjusting the strength had little effect on the overall classification accuracies.
%
We consider this insensitivity to be a significant strength of this approach, as the model is able to apply enough pressure to the latent space to obtain high classification accuracies without having to hand tune parameter values.

%
For the datapoints without labels, we can again perform variational inference, treating the labels as random variables.
%
Specifically, the unsupervised objective, $\mathcal{L}_{\acrshort{ReVAE}}(\x)$, derives as the standard (unsupervised) \gls{ELBO}.
%
However, it requires marginalising over labels as $p(\z) = p(\z_c)p(\z_{\backslash c}) = p(\z_{\backslash c})\sum_{\y} p(\z_c  |  \y) p(\y)$.
This can be computed exactly, but doing so can be prohibitively expensive if the number of possible label combinations is large.
%
In such cases, we apply Jensen's inequality a second time to the expectation over $\y$ (see~\cref{app:alt-elbo}) to produce a looser, but cheaper to calculate, \gls{ELBO} given as
%
\begin{align}
	\mathcal{L}_{\acrshort{ReVAE}}(\x) &=E_{\qzx\qyz}\left[\log \left(\frac{\pxz p_\psi(\z  \mid  \y)  p(\y)}{\qyz\qzx}\right)\right].
	\label{eq:unsup-revae_p}
\end{align}
%
Combining \cref{eq:sup-revae} and \cref{eq:unsup-revae_p}, we get the following lower bound on the log probability of the data
%
\begin{align}
   \log p\left(\mathcal{D}\right)
  \geq \sum\nolimits_{(\x, \y)\in \sD} \mathcal{L}_{\gls{ReVAE}}(\x, \y)
  + \sum\nolimits_{\x\in \uD} \mathcal{L}_{\gls{ReVAE}}(\x),
\end{align}
%
that unlike prior approaches faithfully captures the variational free energy of the model.
%
As shown in \cref{sec:experiments}, this enables a range of new capabilities and behaviors to encapsulate label characteristics.
%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../rep_vae_iclr"
%%% End:


==> sections/rethink.tex <==
% !TEX root =  rep_vae_iclr.tex

As we explained in the last section, the de facto assumption for most approaches to supervision in \glspl{VAE} is that the labels correspond to a partially observed augmentation of the latent space, $\zy$.
%
However, this can cause a number of issues if we want the latent space to encapsulate not just the labels themselves, but also the characteristics \emph{associated} with these labels.
%
For example, encapsulating the youthful characteristics of a face, not just the fact that it is a ``young'' face.
%
At a abstract level, such an approach fails to capture the relationship between the inputs and labels: it fails to isolate characteristic information associated with each label from the other information required to reconstruct data.
%
More specifically, it fails to deal with the following issues.

Firstly, the information in a datapoint associated with a label is richer than stored by the (typically categorical) label itself.
%
That is not to say such information is absent when we impose $\zy=\y$, but here it is \emph{entangled} with the other latent variables $\zny$, which simultaneously contain the associated information for \emph{all} the labels.
%
Moreover, when $\y$ is categorical, it can be difficult to ensure that the \gls{VAE} actually uses $\zy$, rather than just capturing information relevant to reconstruction in the higher-capacity, continuous, $\zny$.
%
Overcoming this is challenging and generally requires additional heuristics and hyper-parameters.

Second, we may wish to manipulate characteristics without fully changing the categorical label itself.
%
For example, making a CelebA image depict more or less `smiling' without fully changing its \texttt{``smile''} label.
%
Here we do not know how to manipulate the latents to achieve this desired effect: we can only do the binary operation of changing the relevant variable in $\zy$.
%
Also, we often wish to keep a level of diversity when carrying out conditional generation and, in particular, interventions.
%
For example, if we want to add a smile, there is no single correct answer for how the smile would look, but taking $\zy=\texttt{"smile"}$ only allows for a single point estimate for the change.
%

Finally, taking the labels to be explicit latent variables can cause a mismatch between the VAE prior $p(\z)$ and the pushforward distribution of the data to the latent space $q(\z) = \E_{p_{\mathcal{D}}(\x)}[\qzx]$.
%
During training, latents are effectively generated according to $q(\z)$, but once learned, $p(\z)$ is used to make generations; variations between the two effectively corresponds to a train-test mismatch.
%
As there is a ground truth data distribution over the labels (which are typically not independent), taking the latents as the labels themselves implies that there will be a ground truth $q(\zy)$.
%
However, as this is not generally known a priori, we will inevitably end up with a mismatch.
%

\paragraph{What do we want from supervision?}
Given these issues, it is natural to ask whether having latents directly correspond to labels is actually necessary.
%
To answer this, we need to
%
think about exactly what it is we are hoping to achieve through the supervision itself.
%
Along with uses of \glspl{VAE} more generally, the three most prevalent tasks are:
%
\textbf{a) Classification}, predicting the labels of inputs where these are not known a priori;
%
\textbf{b) Conditional Generation}, generating new examples conditioned on those examples conforming to certain desired labels; and
%
\textbf{c) Intervention}, manipulating certain desired characteristics of a data point before reconstructing it.

Inspecting these tasks, we see that for classification we need a classifier form $\z$ to $\y$, for conditional generation we need a mechanism for sampling $\z$ given $\y$, and for inventions we need to know how to manipulate $\z$ to bring about a desired change.
%
None of these require us to have the labels directly correspond to latent variables.
%
Moreover, as we previously explained, this assumption can be actively harmful, such as restricting the range of interventions that can be performed.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../rep_vae_iclr"
%%% End:

